Digital Life Project: Autonomous 3D Characters with Social Intelligence

In this work, we present Digital Life Project, a framework utilizing language as the universal medium to build autonomous 3D characters, who are capable of engaging in social interactions and expressing with articulated body motions, thereby simulating life in a digital environment. Our framework comprises two primary components: 1) SocioMind: a meticulously crafted digital brain that models personalities with systematic few-shot exemplars, incorporates a reflection process based on psychology principles, and emulates autonomy by initiating dialogue topics; 2) MoMat-MoGen: a text-driven motion synthesis paradigm for controlling the character's digital body. It integrates motion matching, a proven industry technique to ensure motion quality, with cutting-edge advancements in motion generation for diversity. Extensive experiments demonstrate that each module achieves state-of-the-art performance in its respective domain. Collectively, they enable virtual characters to initiate and sustain dialogues autonomously, while evolving their socio-psychological states. Concurrently, these characters can perform contextually relevant bodily movements. Additionally, a motion captioning module further allows the virtual character to recognize and appropriately respond to human players' actions. Homepage: https://digital-life-project.com/

==> figures/applications.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/images/applications.pdf}
    \caption{Applications (Placeholder)}
    \label{fig:applications}
\end{figure*}

==> figures/momat-mogen.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/images/momat-mogen.pdf}
    \caption{\textbf{\body}}
    \label{fig:momat-mogen}
\end{figure*}

==> figures/reflection.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/images/reflection.pdf}
    \caption{Reflection Raw}
    \label{fig:reflection}
\end{figure}

==> figures/teaser_old.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/images/teaser_old.pdf}
    \caption{Pipeline Raw}
    \label{fig:overall_pipeline}
\end{figure*}

==> figures/visual_mogen.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/images/visual_mogen.pdf}
    \caption{Visualization of MoGen (Placeholder, use smplx).}
    \label{fig:visual_mogen}
\end{figure}
